Coupled Diffusion Sampling for Training-Free Multi-View Image Editing

We present an inference-time diffusion sampling method to perform multi-view consistent image editing using pre-trained 2D image editing models. These models can independently produce high-quality edits for each image in a set of multi-view images of a 3D scene or object, but they do not maintain consistency across views. Existing approaches typically address this by optimizing over explicit 3D representations, but they suffer from a lengthy optimization process and instability under sparse view settings. We propose an implicit 3D regularization approach by constraining the generated 2D image sequences to adhere to a pre-trained multi-view image distribution. This is achieved through coupled diffusion sampling, a simple diffusion sampling technique that concurrently samples two trajectories from both a multi-view image distribution and a 2D edited image distribution, using a coupling term to enforce the multi-view consistency among the generated images. We validate the effectiveness and generality of this framework on three distinct multi-view image editing tasks, demonstrating its applicability across various model architectures and highlighting its potential as a general solution for multi-view consistent editing.

==> tables/magic_fixup_table.tex <==
\begin{table}[t]
\centering
\vspace{-30pt}
\caption{Quantitative comparison on spatial editing. We evaluate our method against GT renders of the target edit, and measure the geometric consistency with MEt3r. In our user studies, our method is preferred by a large margin. For reference, we include the metrics for independent per-image editing and single image-to-MV baselines.}
\label{tab:spatial_edit}
\begin{tabular}{l|ccccc }
\toprule
& \multicolumn{3}{c}{Per-image metrics} & MV metric & \\
\cmidrule(lr){2-4} \cmidrule(lr){5-5}
Method & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & MEt3r $\downarrow$ & User pref. $\uparrow$ \\
\midrule
Per-image \citep{alzayer2025magicfixup}& 16.5 & 0.550 & 0.253 & 0.353 & - \\
Image-to-MV \citep{zhou2025seva} & 12.84 & 0.400 & 0.556 & 0.417 & - \\
\midrule
\cite{liu2022compositional} & 16.5 & 0.530 & \textbf{0.354} & 0.368 & 9\% \\
\cite{yilun2023reuse} & 16.7 & 0.548 & 0.411 & 0.344 & 1\% \\
SDEdit \citep{meng2022sdedit} & 15.4 & 0.458 & 0.468 & 0.393 & 11\% \\
\textbf{Coupled Sampling (Ours)} & \textbf{17.0} & \textbf{0.550} & 0.421 & \textbf{0.335} & \textbf{80\%} \\
\bottomrule
\end{tabular}
\vspace{-5pt}
\end{table}

==> tables/t2mv_table.tex <==
\begin{table}[t]
\centering
\caption{Comparison of sampling methods across different Stable Diffusion backbones on the alignment between text conditioning and generated samples. Higher CLIP Score and VQA Score indicate better performance, while lower MEt3r is better.}
\label{tab:sd_comparison}
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{3}{c}{\textbf{Stable Diffusion 2.1}} & \multicolumn{3}{c}{\textbf{Stable Diffusion XL}} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}
Method & CLIP $\uparrow$ & VQA $\uparrow$ & MEt3r $\downarrow$ & CLIP $\uparrow$ & VQA $\uparrow$ & MEt3r $\downarrow$ \\
\midrule
2D Sampling & 33.33 & 00.00 & 0.000 &  33.36 & 00.00 & 0.000 \\
Multiview Sampling & 30.32 & 00.00 & 0.000 & 32.01 & 00.00 & 0.000 \\
Our Sampling & 32.07 & 00.00 & 0.000 & 32.82 & 00.00 & 0.000 \\
\bottomrule
\end{tabular}
\end{table}
